COOPER: Coordinating Specialized Agents towards a Complex Dialogue Goal

In recent years, there has been a growing interest in exploring dialogues with more complex goals, such as negotiation, persuasion, and emotional support, which go beyond traditional service-focused dialogue systems. Apart from the requirement for much more sophisticated strategic reasoning and communication skills, a significant challenge of these tasks lies in the difficulty of objectively measuring the achievement of their goals in a quantifiable way, making it difficult for existing research to directly optimize the dialogue procedure towards them. In our work, we emphasize the multifaceted nature of complex dialogue goals and argue that it is more feasible to accomplish them by comprehensively considering and jointly promoting their different aspects. To this end, we propose a novel dialogue framework, Cooper, which coordinates multiple specialized agents, each dedicated to a specific dialogue goal aspect separately, to approach the complex objective. Through this divide-and-conquer manner, we make complex dialogue goals more approachable and elicit greater intelligence via the collaboration of individual agents. Experiments on persuasion and emotional support dialogues demonstrate the superiority of our method over a set of competitive baselines.

==> sections/Introduction_backup.tex <==
\section{Introduction}

The use of human language is intentional and purposeful \cite{austin1975things,gricelogic}. %speech act theory, Grice's theory of implicatures, Relevance Theory
In daily communication, we use language deliberately to achieve various goals, ranging from simple inquiries about a product's pricing to complex objectives like resolving conflicts. 
%Goal-oriented dialogues are also an important AI research area that has been investigated for decades. 
Developing goal-oriented dialogue systems has also been a prominent research topic. % that has been investigated for decades. 
%In the field of automatic dialogue systems, goal-oriented dialogues are also an important research area that has been investigated for decades. 
%In the early research, extensive efforts have been made to realize systems that can offer customer services like helping users with ticket booking, restaurant reservation, etc \red{[cite]}. %appointment scheduling, etc. 
%These systems, more commonly referred to as ``task-oriented dialogue systems", \blue{are designed for very specific and tangible goals, only involved with one single task at a time}. 
%In this domain, most early efforts were directed to service-focused task-oriented systems that can assist users with ticket booking, restaurant reservation, etc \cite{wen-etal-2017-network, budzianowski-etal-2018-multiwoz, hosseini2020simple}.
%The goals of such systems are very specific and narrowly defined .% \red{[Comment: use some old references]}. 
In the past few years, there has been increasing research interest in dialogue tasks with more complex goals, such as persuasion \cite{wang-etal-2019-persuasion, sanders2022towards}, negotiation \cite{he2018decoupling, zhan2022let}, and emotional support \cite{liu2021towards}, which extend beyond the traditional service-focused dialogue systems (e.g. for assisting with ticket booking or restaurant reservation) \cite{rieser2005implications, boyer2011affect, wen2016network}. %(e.g. for assisting with ticket booking or restaurant reservation)
These dialogues possess goals that are more general and less tangible. 

Typically, such a complex dialogue goal is multifaceted, encompassing multiple aspects to jointly work towards the broad objective. 
For instance, in an Emotional Support Conversation (ESC), the psychological guidelines suggest that effective emotional support should include three aspects:\footnote{We notice that some works refer to the ``\emph{aspects}'' here as ``\emph{stages}'', but they also emphasize that these ``stages'' are closely interwoven in practice rather than sequential  \cite{hill2009helping,liu2021towards}. Given that, we choose to call them as ``aspects'' uniformly in our work to avoid misunderstanding about their sequential nature. } \emph{exploration} (identify the support-seeker's problem), \emph{comforting} (comfort the seeker's emotion through expressing empathy), and \emph{action} (help the seeker solve the problem) \cite{liu2021towards}. %, which generally refers to the preconditions for a broad dialogue goal,
%In our daily lives, when we want to accomplish a complex dialogue goal, such as ``facilitating a constructive conversation with a colleague about a sensitive work-related issue without causing any tension'', usually, we would conceive a sketchy plan which divides that broad goal into several stages. 
%For instance, one might start by creating a conducive environment, actively listening to the colleague's perspective, and respectfully presenting the concerns. 
%For instance, when faced with a sensitive work-related issue in our daily lives, we might want to facilitate a constructive conversation with a colleague without causing any tension. 
%To achieve this complex dialogue goal, usually, we would conceive a sketchy plan which divides that broad goal into several stages, like starting by creating a conducive environment, then actively listening to the colleague's perspective, and respectfully presenting our concerns.   
%\blue{More generally, in our daily life, when we want to accomplish a complex dialogue goal, such as ``cautiously reminding your adolescent daughter that her new boyfiend might not be a good person'', usually, we would also conceive a sketchy plan which divides the broad goal into several stages.} For instance, one might start by casually gossipping with the daughter to create a warm atmosphere, followed by actively listening and displaying genuine interest in her life, and then respectfully sharing some observations with her.
%In practice, these ``\emph{stages}'' are interwoven with each other rather than strictly sequential, which requires flexible arrangement according to the context \cite{hill2009helping}. This is also the case with other CGOD scenarios. Given that, we would refer to them as the ``\emph{aspects}'' instead of ``\emph{stages}'' within the broad dialogue objective hereafter to avoid misunderstanding about the sequential nature. 
%\blue{though there exists particular interdependence among these ``\emph{stages}''}
%These stages can be regarded as the aspects within the broad goal of ESC, as, in practice, they are interweaved with each other rather than strictly sequential. Their order should be flexibly determined according to the context. 
%such as ``cautiously reminding your adolescent daughter that her new boyfiend might not be a good person'', usually, 
%Take the Emotional Support Conversation (ESC) as an example. The psychological guidelines suggest that an ESC should include three stages to achieve emotional support: exploration (identify the problem), comforting (comfort the seeker's emotion through expressing empathy), and action (\blue{help the seeker solve the problem}) \red{[cite]}.
%Consider a complex dialogue goal, such as facilitating a constructive conversation with a colleague about a sensitive work-related issue, without causing tension or conflict. In such cases, a strategic approach typically involves creating a conducive environment, actively listening to their perspective, and respectfully presenting your observations or concerns.
%In a CGOD, the interlocutor needs to conduct intensive reasoning to determine which aspect to prioritize at each point through the conversation. During this reasoning process, it is essential to cautiously consider the interdependence among these aspect. 
Moreover, the aspects within a broad objective are usually interdependent with each other. 
Take the aspects of \emph{exploration} and \emph{comforting} in ESC as an example:  exploring the seeker's situation lays the foundation for conveying appropriate emphy, while comforting the user to be in a better emotional state also makes them more willing to share details about their experiences and feelings. 
%For example, in ESC, the aspect of \emph{exploration} lays the foundation for \emph{comforting}, while \emph{comforting}, which puts the seeker in a better emotional state, can make the seeker more willing to share details about their experiences. 


% did not explicitly consider how to achieve a broad dialogue objective by jointly promote several aspects. Instead, they regard this as one complex task 

Therefore, when determining which aspect to prioritize at each point during the conversation, the interlocutor needs to coordinate the promotion of each aspect with consideration of their interdependence. % and jointly advance them towards the broad objective. %During this reasoning process, it is essential to cautiously consider the interdependence among these aspect. 
%For complex goal-oriented dialogues, sophisticated dialogue \blue{planning} is essential to jointly promote the multiple aspects within the broad objective and adaptively arrange their order. 
This reasoning process requires the interlocutor to dynamically track the state of each aspect and analyze its progression, which involves where the state of this aspect is heading (i.e., its estimated target state at the end of the conversation), and how much progress it has achieved so far. % relative to the expected target (i.e., the estimated distance from the current state to the target). 
For instance, in an ESC, a supporter may capture that it is still necessary to further explore the seeker's situation after analyzing the progression of the aspect \emph{exploration}. 
Simultaneously, considering the current progression of \emph{comforting}, the supporter finds that the seeker might not be ready to pour out more details yet. 
%Coordinating these aspects, the supporter is likely to prioritize promoting the \emph{comforting} aspect in this case.
Coordinating these aspects, the supporter is very likely to prioritize promoting the aspect of \emph{comforting} in this case. 
% and \emph{comforting}, the supporter can determine whether it is necessary to further explore the seeker's situation and how much  the support
%\red{[Comment: May be add an example here?]}
%For example, a seasoned emotional supporter can \blue{envision} what problem the seeker is facing and what comforting words they may need according to their experience, even long before the conversation ends.  
% and making adaptive adjustments throughout the conversation. %\red{[Comment: What is ``progression''? Do we need more illustration here as in the \emph{progression-aware} paper?]} 

However, existing research simply regarded the complex dialogue goal as one broad task to optimize the dialogue procedure, without explicitly considering the aspects within it or the interdependence among these aspects \cite{zhou2019augmenting, joshi2021dialograph, cheng2022improving, chen-etal-2023-controllable}. 
Even by leveraging the modern Large Language Models (LLMs), these methods demonstrate very limited awareness of the overall dialogue progression and tend to repeatedly adopt similar dialogue strategies that focus on promoting one aspect within the broad goal while neglecting the others. 
As in ESC, \citet{zhao2023chatgpt} showed that the LLM-based ESC system often continuously giving coping suggestions to the user, largely overlooking the important process of exploration and comforting. 
%inquiring about additional details regarding their situation and expressing empathy to comfort their emotion. 
\begin{comment}
This can be challenging even for humans without particular training and abundant experience \red{[cite]}. %\red{[Comment: still lack a one-sentence clear summarization of the challenge.]} %, so they are \blue{usually interweaved with each other} rather than strictly sequential. 
Recent works applied modern Large Language Models (LLM) to complex goal-oriented dialogues by directly prompting the LLM to generate the utterance \cite{zhao2023chatgpt} or further improving the performance via iterative revision \cite{fu2023improving}. They exhibited remarkable improvement compared to the previous methods, \blue{especially in terms of the coherence between the generated utterance with the context}. However, a significant limitation of these LLM-based methods is that they tend to passively respond to the interlocutor, without a larger picture of the overall dialogue progression in mind \red{[cite]} . %rather than cautiously advancing the aspects within the broad objective with a larger picture of the overall dialogue progression in mind. 
For example, when dealing with the task of ESC, they often continuously offer coping suggestions to the user, overlooking the important process of inquiring about additional details regarding their situation and expressing empathy to comfort their emotion \red{[cite]}. 
%Instead, they tend to passively respond to the interlocutor at each turn without consideration of the dialogue progression. 
\end{comment}

In this paper, we propose a novel dialogue framework, \textsc{Cooper}, which coordinates multiple specialized agents that separately deal with different aspects within a complex dialogue goal to jointly approach the broad objective. Specifically, each agent is designed to exclusively focus on the relevant part of the dialogue context associated with its assigned aspect. By tracking the current state of the assigned aspect, the agent analyzes its progression and suggests several topic candidates to be mentioned in the next utterance that can further promote the aspect (e.g. the agent responsible for the aspect of \emph{exploration} will suggest several questions to ask the seeker). %This signal \blue{should} indicate where the \blue{state} of this aspect is heading, i.e., the estimated \blue{target} state at the end of conversation, and how far the dialogue is away from the target currently.\footnote{\red{By ``state'', we refer to the summarization of ... By ``target'', we do not mean a specific achievement state of a dialogue goal as in traditional task-oriented dialogues. Instead, we refer to ... }} At the same time, each agent needs to suggest several topic candidates for the next utterance to advance the assigned aspect.  
%analyze the current progression of the aspect and consider how to further promote it. ore concretely, it is responsible for producing a progression signal indicates where the state of this aspect is heading, i.e., the estimated target state at the end of conversation, and how far the dialogue is away from the target.  and suggesting several topic candidates for the next utterance to advance the assigned aspect. This progression signal indicates where the state of this aspect is heading, i.e., the estimated target state at the end of conversation, and how far the dialogue is away from the target. 
Then, we coordinate these specialized agents by ranking their suggested topic candidates with global consideration of the overall dialogue progression. Finally, the top-ranked topic candidates are fused to guide the generation of the next utterance. %\red{[Comment: Maybe more discussion on the advantages of the proposed approach, like why such a divide-and-conquer manner is more applicable in this scenario. ]}

We use the task of ESC and persuasion dialogues as the testbed of our framework, where our method demonstrates significant improvement compared with a set of competitive baselines. In summary, our contributions are as follows:%\blue{Extensive experiments show the effectiveness of our proposed approach.} 
\begin{itemize}
    \item To this best of knowledge, this is the first work that explores how to achieve a complex dialogue goal by explicitly modelling its multiple aspects and jointly promoting them with consideration of their interdependence. %\red{[Comment: How about previous works? How do they achieve a complex dialogue goal?What's the difference? Not mentioned above. Maybe it should be added to the third paragraph. ]}
    \item We propose \textsc{Cooper}, an innovative framework that employs coordination among specialized agents to jointly approach a complex dialogue goal.
    \item Extensive experiments demonstrate the effectiveness of our approach and reveal the limitations of current LLMs in handling complex dialogue goals. 
\end{itemize}

%\textbf{\underline{Coo}}rdination of s\textbf{\underline{p}}ecialized ag\textbf{\underline{e}}nts for complex goal-o\textbf{\underline{r}}iented dialogues.


==> sections/Introduction_backup3.tex <==
\section{Introduction}

The use of human language is intentional and purposeful \cite{austin1975things,gricelogic}. 
In daily communication, we use language deliberately to achieve various goals, ranging from simple inquiries about a product's pricing to complex objectives like resolving conflicts. 
Developing goal-oriented dialogue systems has also been a prominent research topic. 

In recent years, there has been growing research interest in dialogue tasks with more complex objectives, such as persuasion \cite{wang-etal-2019-persuasion}, negotiation \cite{he2018decoupling}, and emotional support \cite{liu2021towards}. 
Compared to traditional service-focused goal-oriented dialogue systems \cite{rieser2005implications, boyer2011affect, wen2016network}, these tasks require much more sophisticated strategic reasoning and communication skills. 
Moreover, another significant challenge lies in the difficulty of objectively measuring the achievement of such complex dialogue goals in a quantifiable and reliable way.  
Consequently, most existing research stays overly focused on how to fit the ground-truth data, without explicit consideration of how each utterance could contribute to the final objective \cite{zhou-etal-2019-dynamic, joshi2021dialograph, chen-etal-2023-controllable}. In the few works that attempt to model these dialogue goals explicitly, it remains highly challenging to optimize the dialogue procedure towards them directly due to their inherent intangibility \cite{cheng2022improving, zhou-etal-2023-facilitating}. Recent studies show that even state-of-the-art Large Language Models (LLMs) struggle with with these tasks, exhibiting weak awareness of the overall dialogue progression and often producing similar content repeatedly \cite{zhao2023chatgpt}. %often producing similar content repeatedly and failing to accomplish a complex dialogue goal through multiple interactions strategically \cite{zhao2023chatgpt}. 

%These dialogues possess goals that are more general and less tangible. 
% and argue that it is more feasible to accomplish them by comprehensively considering and jointly promoting their different aspects
In our work, we highlight the multifaceted nature of complex dialogue goals, which typically encompass multiple interdependent aspects that must be collectively promoted to approach the final objective. 
For instance, psychological guidelines suggest that Emotional Support Conversations (ESC) should include three key aspects:\footnote{Some works may refer to the ``{aspects}'' here as ``{stages}'', but they also emphasize that these ``stages'' are closely interwoven in practice rather than sequential  \cite{liu2021towards}. Given that, we choose to call them as ``aspects'' uniformly in our work to avoid misunderstanding about their sequential nature. } \emph{exploration} (identify the support-seeker's problem), \emph{comforting} (comfort the seeker's emotion through expressing empathy), and \emph{action} (help the seeker solve the problem)  \cite{hill2009helping}. 
These aspects are interdependent. As in ESC, exploring the seeker's situation lays the foundation for comforting the seeker's emotion, which in turn makes them more willing to share details about their experiences and feelings. % while comforting the user to be in a better emotional state makes them more willing to share details about their experiences and feelings. 

%Compared with directly optimizing towards the complex dialogue goal, it is more approachable to accomplish them by comprehensively considering and jointly promoting their different aspects. 
To address the challenge of complex goal modeling and overcome the limitations of existing LLM-based methods on these tasks, we propose a novel dialogue framework, \textsc{Cooper}. It coordinates multiple specialized agents, which separately focus on different dialogue goal aspects, to approach a complex objective. Specifically, each agent is designed to conduct a \emph{local analysis} of the designated aspect, which involves summarizing its current state and proposing several topic candidates for the next utterance that can further promote it. For instance, the agent responsible for the \emph{exploration} aspect in ESC will summarize the seeker's situation and suggest questions to ask the seeker. Then, \emph{global coordination} is conducted by ranking all the topic candidates, which will be further elaborated later. Finally, we use the top-ranked ones to guide the utterance generation. 

In this framework, the two tasks involved in local analysis, text summarization and generating brief content on a specified subject, have proved empirically achievable for current LLMs. Through this divide-and-conquer manner, we make the complex goal more approachable and aim to elicit greater intelligence via the collaboration of individual agents. The major challenge here remains in the step of global coordination. 

In \textsc{Cooper}, we develop global coordination based on the insight that this process is similar to the one conducted by real-life interlocutors, who must strategically coordinate the priority of different dialogue goal aspects due to their interdependence. 
To achieve this, they need to comprehensively consider the progression of all the aspects, which involves measuring their progress and anticipate their directions. \blue{As in the case of ESC, a seasoned supporter must continuously analyze the current knowledge of the seeker's situation and estimate the underlying root problem for further exploration. They would also monitor the progression of the \emph{comforting} and \emph{action} aspects simultaneously in order to determine which aspect to prioritize at each point of the conversation. }
Based on this insight, we develop a progression analysis module for each dialogue aspect in \textsc{Cooper}, which produces a progression signal that is designed to indicate how much progress has been achieved so far regarding this aspect and its estimated target state at the end of the conversation. By comprehensively consider all the progression signals, \textsc{Cooper} conducts global coordination among the specialized agents by ranking their suggested topic candidates. % and finally, uses the the top-ranked ones to guide the utterance generation.
%Then, we coordinate the specialized agents by ranking all the topic candidates with consideration of the overall dialogue progression. Finally, the top-ranked topic candidates are used to guide the generation of the next utterance. 

Experiments on ESC and persuasion dialogues demonstrate the superiority of \textsc{Cooper} over a set of competitive LLM-based methods and previous state-of-the-art.
In summary, our contributions are as follows:%\blue{Extensive experiments show the effectiveness of our proposed approach.} 
\begin{itemize}
    \item To this best of knowledge, this is the first work that explores how to achieve a complex dialogue goal by coordinating the joint promotion of its different aspects. 
    \item We propose \textsc{Cooper}, an innovative framework that coordinates multiple specialized agents to collaboratively work towards a complex dialogue goal.
    \item Extensive experiments demonstrate the effectiveness of our approach and also reveal the limitations of current LLMs in handling complex dialogue goals. 
\end{itemize}

%\textbf{\underline{Coo}}rdination of s\textbf{\underline{p}}ecialized ag\textbf{\underline{e}}nts for complex goal-o\textbf{\underline{r}}iented dialogues.


==> sections/Introduction_backup4.tex <==
\section{Introduction}

The use of human language is intentional and purposeful \cite{austin1975things,gricelogic}. 
In daily communication, we use language deliberately to achieve various goals, ranging from simple inquiries about a product's pricing to complex objectives like resolving conflicts. 
Developing goal-oriented dialogue systems has also been a prominent research topic. 

In recent years, there has been growing research interest in dialogue tasks with more complex objectives, such as persuasion \cite{wang-etal-2019-persuasion}, negotiation \cite{he2018decoupling}, and emotional support \cite{liu2021towards}. 
Compared to traditional service-focused goal-oriented dialogue systems \cite{rieser2005implications, boyer2011affect, wen2016network}, these tasks require much more sophisticated strategic reasoning and communication skills. 
Recent studies show that even state-of-the-art Large Language Models (LLM) struggle with with these tasks, where they exhibit weak awareness of the overall dialogue progression and fail to accomplish the complex goal strategically through multiple interactions  \cite{zhao2023chatgpt}.
Moreover, another significant challenge lies in the difficulty of objectively measuring the achievement of such complex dialogue goals in a quantifiable and reliable way.  
Consequently, most existing research stays overly focused on how to fit the ground-truth data, without explicit consideration of how each utterance could contribute to the final objective \cite{zhou-etal-2019-dynamic, joshi2021dialograph}. In the few works that attempt to model these dialogue goals explicitly, it remains highly challenging to optimize the dialogue procedure towards them directly due to their inherent intangibility \cite{cheng2022improving, zhou-etal-2023-facilitating}. 
%Despite the powerful capabilities demonstrated lately by Large Language Models (LLMs),  %often producing similar content repeatedly and failing to accomplish a complex dialogue goal through multiple interactions strategically \cite{zhao2023chatgpt}. 

%These dialogues possess goals that are more general and less tangible. 
% and argue that it is more feasible to accomplish them by comprehensively considering and jointly promoting their different aspects
In this work, we highlight the multifaceted nature of complex dialogue goals, which typically encompass multiple interdependent aspects that must be collectively promoted to approach the final objective. 
For instance, psychological guidelines suggest that Emotional Support Conversations (ESC) should include three key aspects:\footnote{Some works may refer to the ``{aspects}'' here as ``{stages}'', but they also emphasize that these ``stages'' are closely interwoven in practice rather than sequential  \cite{liu2021towards}. Given that, we choose to call them as ``aspects'' uniformly in our work to avoid misunderstanding about their sequential nature. } \emph{exploration} (identify the support-seeker's problem), \emph{comforting} (comfort the seeker's emotion through expressing empathy), and \emph{action} (help the seeker solve the problem)  \cite{hill2009helping}. 
These aspects are interdependent, just as exploring the seeker's situation lays the foundation for comforting the seeker's emotion, which in turn makes them more willing to share details about their experiences. 
Due to this interdependence, the interlocutor must strategically coordinate the priority of different aspects during the conversation. This requires them to comprehensively consider the progression of all the aspects, which involves measuring their progress and anticipate their directions. As in ESC, a seasoned supporter must continuously analyze the current knowledge of the seeker's situation and estimate the underlying root problem for further exploration. They also need to monitor the states of the \emph{comforting} and \emph{action} aspects simultaneously, in order to determine which aspect to prioritize at each point of the conversation.  

%Compared with directly optimizing towards the complex dialogue goal, it is more approachable to accomplish them by comprehensively considering and jointly promoting their different aspects. 
Based on the above insight, we propose a novel dialogue framework, \textsc{Cooper}, to address the challenge of complex goal modeling and transcend the limitations of existing LLM-based methods, It coordinates multiple specialized agents, which separately focus on different dialogue goal aspects, to approach a complex dialogue goal. 
For each agent, it is responsible for summarizing the current state of its assigned aspect and generating several topic candidates for the next utterance that can further promote this aspect. For example, the agent responsible for the \emph{exploration} aspect in ESC will summarize the seeker's situation and suggest questions to ask the seeker. 
Besides, each agent also includes a progression analysis module. It is designed to produce a progression signal, indicating how much progress has been achieved so far regarding the designated aspect and its estimated target state at the end of the conversation. 
By comprehensively consider all the progression signals, \textsc{Cooper} conducts global coordination among the specialized agents by ranking their suggested topic candidates. 
Finally, the top-ranked candidates are used to guide the utterance generation. 

%In this framework, the two tasks involved in the specialized agent, text summarization and generating brief content on a specified subject, have proved empirically achievable for current LLMs. 
Through this divide-and-conquer manner, we make the complex goal more approachable and elicit greater intelligence via the collaboration of individual agents. 
Experiments on ESC and persuasion dialogues demonstrate the superiority of \textsc{Cooper} over a set of competitive LLM-based methods and previous state-of-the-art.
In summary, our contributions are as follows:%\blue{Extensive experiments show the effectiveness of our proposed approach.} 
\begin{itemize}
    \item To this best of knowledge, this is the first work that explores how to achieve a complex dialogue goal by coordinating the joint promotion of its different aspects. 
    \item We propose \textsc{Cooper}, an innovative framework that coordinates multiple specialized agents to collaboratively work towards a complex dialogue goal.
    \item Extensive experiments demonstrate the effectiveness of our approach and also reveal the limitations of current LLMs in handling complex dialogue goals. 
\end{itemize}

%\textbf{\underline{Coo}}rdination of s\textbf{\underline{p}}ecialized ag\textbf{\underline{e}}nts for complex goal-o\textbf{\underline{r}}iented dialogues.

